Confidence Matters: Revisiting Intrinsic Self-Correction Capabilities of Large Language Models

The recent success of Large Language Models (LLMs) has catalyzed an increasing interest in their self-correction capabilities. This paper presents a comprehensive investigation into the intrinsic self-correction of LLMs, attempting to address the ongoing debate about its feasibility. Our research has identified an important latent factor - the "confidence" of LLMs - during the self-correction process. Overlooking this factor may cause the models to over-criticize themselves, resulting in unreliable conclusions regarding the efficacy of self-correction. We have experimentally observed that LLMs possess the capability to understand the "confidence" in their own responses. It motivates us to develop an "If-or-Else" (IoE) prompting framework, designed to guide LLMs in assessing their own "confidence", facilitating intrinsic self-corrections. We conduct extensive experiments and demonstrate that our IoE-based Prompt can achieve a consistent improvement regarding the accuracy of self-corrected responses over the initial answers. Our study not only sheds light on the underlying factors affecting self-correction in LLMs, but also introduces a practical framework that utilizes the IoE prompting principle to efficiently improve self-correction capabilities with "confidence". The code is available at https://github.com/MBZUAI-CLeaR/IoE-Prompting.git.

==> figures/prompts.tex <==
\begin{figure}
	\centering
	\tiny
	\begin{tcolorbox}[enhanced, arc=3mm, colback=gray!10!white, boxrule=0pt, boxsep=1pt,colframe=gray!50!white,  boxed title style={colback=gray!90!white}, boxed title style= {boxrule=2pt, boxsep=2pt}, attach boxed title to top left={yshift=-2mm, xshift=2mm}, title=\textbf{[P1] Standard Prompt}  
		]
		\includegraphics[width=0.9em]{figures/user_icon.png} : \textcolor{mycolor}{John plans to sell all his toys and use the money to buy video games. He has 13 lego sets and he sells them for \$15 each. He ends up buying 8 video games for \$20 each and has \$5 left. How many lego sets does he still have?  Explain your reasoning. Explain your reasoning.} \\
		\includegraphics[width=0.9em]{figures/llm_icon.png} :  \textcolor{second}{... Therefore, he still has 11 lego sets.} \textcolor{wrongcolor}{\textbf{(Incorrect)}}
	\end{tcolorbox}

\begin{tcolorbox}[enhanced, arc=3mm, colback=gray!10!white, boxrule=0pt, boxsep=1pt,colframe=gray!50!white,  boxed title style={colback=gray!90!white}, boxed title style= {boxrule=2pt, boxsep=2pt}, attach boxed title to top left={yshift=-2mm, xshift=2mm}, title=\textbf{[P2] IoE-based Prompts}
	]
	\includegraphics[width=0.9em]{figures/user_icon.png} : \textcolor{mycolor}{If you are very confident about your answer, maintain your answer. Otherwise, update your answer.} \\
	\includegraphics[width=0.9em]{figures/llm_icon.png} :  \textcolor{second}{I made a mistake in my previous response. ... Therefore, he still has 2 lego sets.} \textcolor{rightcolor}{\textbf{(Correct)}}
\end{tcolorbox}

\begin{tcolorbox}[enhanced, arc=3mm, colback=gray!10!white, boxrule=0pt, boxsep=1pt,colframe=gray!50!white,  boxed title style={colback=gray!90!white}, boxed title style= {boxrule=2pt, boxsep=2pt}, attach boxed title to top left={yshift=-2mm, xshift=2mm}, title=\textbf{[Opional P3] Decision Prompt}
	]
	\includegraphics[width=0.9em]{figures/user_icon.png} : \textcolor{mycolor}{You give two different answers in previous responses. Check the problem and your answers again, and give the best answer.} \\
	\includegraphics[width=0.9em]{figures/llm_icon.png} :  \textcolor{second}{Apologies for the confusion. ... Therefore, he still has 2 lego sets.} \textcolor{rightcolor}{\textbf{(Correct)}}
\end{tcolorbox}
\caption{Example 2 on GSM8K \cite{cobbe2021training} with \texttt{gpt-3.5-turbo-1106}, using our proposed three-step IoE-based prompts. Refer to Section \ref{sec3:ioe} and Appendix for more details.}
\label{fig:prompts}
\end{figure}
